When Prompts Ignore Structure: Graph-Based Attribute Reasoning for Calibrated VLMs

Reliable confidence estimation remains a key limitation of test-time adaptation in vision-language models (VLMs), where prompt tuning improves zero-shot accuracy but often degrades calibration due to entropy-driven overconfidence. Prior approaches mitigate this using LLM-derived class attributes and contrastive regularization, yet treat attributes independently, ignoring their relational structure. We propose ARGTCA, which represents (class, attribute) pairs as nodes in a Symbolic Attribute Graph and trains a Graph Attention Network (GAT) using contrastive objectives to produce structurally informed embeddings that capture inter-attribute dependencies. We introduce two attribute selection strategies: ARGTCA-DIV for intra-class diversity and ARGTCA-DISC for inter-class discrimination. Experiments across nine benchmarks show that ARGTCA-DIV reduces average Expected Calibration Error (ECE) by approximately ~37% over baselines, while ARGTCA-DISC consistently performs as the second-best variant, reducing average ECE by approximately ~17% over baselines. These results suggest that modeling symbolic attribute interactions provides a principled approach for reliable test-time adaptation in VLMs.

==> 1_intro_v2.tex <==
\section{Introduction}
\label{sec:intro}

Vision-language models (\VLM{}s) such as \CLIP{} \citep{radford2021learning} have shown strong zero-shot image recognition by aligning images and text in a shared embedding space through large-scale contrastive pretraining. \CLIP{} performs zero-shot classification of an image by computing cosine similarities between its visual embedding and class-conditioned text features generated from prompt templates such as \emph{``a photo of a \{class\}''}.  While effective, such templates are suboptimal and domain-agnostic. 
Test-time prompt tuning (\TPT{}) \citep{shu2022test} addresses this by optimizing prompt tokens for each test image using only its own augmented views, with no labeled data. However, \TPT{}s entropy minimization objective inherently drives the model toward overconfident predictions, producing miscalibrated outputs, quantified by the Expected
Calibration Error (\ECE{}) \citep{guo2017calibration}.  It poses a fundamental barrier to deploying \VLM{}s in  safety-sensitive applications such as healthcare diagnostics and autonomous systems, where unreliable uncertainty estimates can have serious consequences. 

\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccc}
        \includegraphics[width=0.30\linewidth]{latex-2/figures/tpt/TPT_Caltech101.png} &
        \includegraphics[width=0.30\linewidth]{latex-2/figures/ctpt/C-TPT-Caltech101.png} &
        \includegraphics[width=0.30\linewidth]{latex-2/figures/tca/tca-Caltech101.png} \\[1pt]
        {\small TPT (4.59)} &
        {\small \CTPT{} (4.24)} &
        {\small \TCA{} (2.56)} \\[4pt]
        \includegraphics[width=0.30\linewidth]{latex-2/figures/otpt/O-TPT-Caltech101.png} &
        \includegraphics[width=0.30\linewidth]{latex-2/figures/atpt/A-TPT_Caltech101.png} &
        \includegraphics[width=0.30\linewidth]{latex-2/figures/argtca/argtca-disc-Caltech101.png} \\[1pt]
        {\small \OTPT{} (3.62)} &
        {\small A-TPT (2.67)} &
        {\small \textbf{Ours} (1.62)} \\
    \end{tabular}
    \caption{Reliability diagrams on Caltech101 dataset (ViT-B/16, \ECE{}($\downarrow$) in parentheses). \TCA{} is overconfident (bars below diagonal); while TPT, \CTPT{}, \OTPT{},
and A-TPT overcorrect into underconfidence (bars above diagonal).
 \ARGTCADisc{} (ours) achieves the closest alignment with the calibration diagonal across all confidence bins. Full results across all datasets are provided in Figure~\ref{fig:reliability-all} in Appendix.}
    \label{fig:reliability-caltech}
\end{figure}
A key insight motivating recent work is that calibration and accuracy are largely \emph{decoupled}: different prompts can achieve nearly identical top-1 accuracy
while exhibiting significantly divergent \ECE{} \citep{yoon2024ctpt}. This implies that the \textit{geometry of the textual feature space}, rather than predictive accuracy alone, governs how well-calibrated a \VLM{}s predictions are. \CTPT{} \citep{yoon2024ctpt} and \OTPT{}\cite{sharifdeen2025otpt} exploit this by adding a feature-dispersion loss and angular dispersion respectively, that spreads class-conditioned text features across the hypersphere. \TCA{} \citep{hebbalaguppe2025tca} complements these geometric objectives by adding \LLM{}-extracted visual attributes for semantically grounded prompt initialization, combined with a contrastive intra-class and inter-class regularization over the resulting text embeddings, achieving strong calibration.
% \insightbox{CLIP classification is governed entirely by cosine similarities between the image vector and class-conditioned text features; it is the geometry of the textual feature space, not predictive accuracy alone, that controls calibration.}
% \insightbox{Classification is entirely driven by angles between the image vector $v$ and each text feature $\hat e_k$. The geometry of the text feature points is what controls calibration.}

\paragraph{Structural limitations of \TCA{}.}
Despite strong calibration performance, \TCA{} exhibits two structural failures that directly degrade the geometry of class-conditioned text features. First, attributes are selected as a flat set based on cosine-similarity without any relational context: on texture-rich datasets such as DTD, attributes such as \textit{rough}, \textit{bumpy}, and \textit{grainy} are nearly collinear in \CLIP{'s}
embedding space, so top-$M'$ selection clusters attribute embeddings tightly and undermines the separation that calibration requires. Second, attributes shared ubiquitously across different classes---such as \textit{mammal} across \textit{leopard}, \textit{dolphin}, and \textit{beaver} in Caltech101---carry diminished discriminative capacity, leaving their embeddings proximate across class boundaries. Both the failure modes are invisible to \TCA{'s} selection procedure, which operates purely on similarity based ordering of LLM generated attributes without any notion of relational geometry between attributes. 

We propose \ARGTCA{} (\textbf{A}ttribute \textbf{R}elation \textbf{G}raph for \textbf{T}est-time \textbf{C}alibration \textbf{A}daptation), a graph-based framework that addresses both structural failures through a Symbolic Attribute Graph (SAG) constructed by representing (class, attribute) pairs as nodes, trained offline via a Graph Attention Network with no task supervision. Two selection strategies derived from the graph — \ARGTCADiv{}{} for intra-class diversity and \ARGTCADisc{}{} for inter-class discrimination. 
% — initialize TCA's prompt tuning at zero additional test-time cost.
% We propose \ARGTCA{} (\textbf{A}ttribute \textbf{R}elation \textbf{G}raph for
% \textbf{T}est-time \textbf{C}alibration \textbf{A}daptation), that addresses both failures  through a graph-based relational framework for attribute selection. We construct a Symbolic Attribute Graph~(\SAG{}) in which $(\text{class, attribute})$ pairs are nodes linked by within-class co-membership and cross-class attribute-sharing edges. A Graph Attention Network~(GAT) propagates relational context across these edges, producing embeddings that capture intra-class complementarity and cross-class redundancy —- properties entirely absent from \TCA{'s} flat-set representation. 
% Two selection criteria emerge from the graph: ARGTCA-DIV for intra-class diversity and ARGTCA-DISC for inter-class discrimination. 
Both strategies operate at zero additional test-time cost — \textbf{Note:} the graph is trained once offline and selection is performed before tuning begins.

We validate \ARGTCA{} across nine benchmark datasets spanning fine-grained recognition, texture classification, and domain-shifted imagery %using both ResNet-50 and ViT-B/16 CLIP backbones.  
% We conduct extensive experiments across nine benchmark datasets and multiple backbone architectures, with systematic ablation studies validating each architectural component. 
% Our results demonstrate that graph-structured relational reasoning over attributes is both necessary and sufficient for consistent calibration improvements. 
and demonstrate empirically that graph-structured relational reasoning over attributes is a key driver of calibration improvement --- as shown in Figure~\ref{fig:reliability-caltech}, \ARGTCA{} produces reliability diagrams most closely aligned with the perfect calibration diagonal, outperforming existing prompt-tuning baselines.
% over \TCA{},  \vinti{figure 1 should be cited here?}.
Our key contributions are:
\begin{itemize}

\item We identify two structural failures in \TCA{}: near-synonymous intra-class
attributes that cluster on the hypersphere, and ubiquitous cross-class attributes that carry no discriminative capacity yet receive no suppression. We construct a Symbolic Attribute Graph~(SAG) from class specific attributes and train a Graph Attention Network via supervised contrastive learning to produce relational embeddings capturing intra-class complementarity and cross-class redundancy.

\item We introduce two selection strategies from graph-refined embeddings:
\ARGTCADiv{}, maximising intra-class semantic complementarity; and \ARGTCADisc{}, maximising distance from all other-class embeddings. Both strategies
operate at zero additional test-time cost and are evaluated across nine benchmarks using CLIP ViT-B/16.

% \item Experiments across nine benchmarks and two CLIP backbones: ResNet50 \& ViT-B16 confirm consistent calibration and accuracy gains over TCA at zero additional test-time cost.
% \item We conduct experiments across nine benchmarks on CLIP with ViT-B/16 backbone to evaluate the graph-informed attribute selection in TCA at zero additional test-time cost.
\end{itemize}
% Our key contributions are as follows:
% \begin{enumerate}
%   \item We identify that \TCA{}'s order-insensitive attribute selection frequently yields near-synonymous, co-occurring attributes that cluster tightly in the CLIP embedding space, undermining the separation necessary for calibration.
%   \item We propose \textbf{\ARGTCA{}}, which reformulates attribute selection as message passing over an attribute--class graph, using a two-layer GAT trained offline to produce neighborhood-aware representations that capture cross-class redundancy and intra-class complementarity.
%   \item We introduce a \emph{relevance--discriminability} criterion instantiated via two complementary strategies: intra-class diversity, maximizing pairwise angular separation among selected attributes, and inter-class discriminability, suppressing attributes shared ubiquitously across classes.
%   \item We conduct extensive experiments across \textcolor{red}{multiple benchmarks and backbones}, confirming that graph-relational structure is the a critical component for calibration improvement, at \textbf{zero additional test-time cost}.
% \end{enumerate}




==> 2_related_work_v2.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Test-Time Adaptation of VLMs}
Foundation models such as \CLIP{}~\citep{radford2021learning, jia2021scaling} enable
zero-shot classification by aligning image and text in a shared embedding space.
While learned prompt methods like CoOp~\citep{zhou2022learning} and
CoCoOp~\citep{zhou2022conditional} improve over hard prompts, they require
labeled data, limiting zero-shot applicability. \TPT{}~\citep{shu2022test}
removes this constraint by adapting prompts via entropy minimization over
augmented views of a single test image, extended further by
DiffTPT~\citep{feng2023diverse} and
PromptAlign~\citep{mirza2024promptalign} through improved augmentation and
distribution alignment. However, entropy minimization drives overconfident
predictions across all \TPT{}-family methods, significantly degrading
calibration relative to the zero-shot baseline\cite{yoon2024ctpt}.
% \subsection{Test-Time Adaptation of VLMs}
% Foundation models for computer vision~\cite{radford2021learning, align}
% align image and text in a shared embedding space, enabling zero-shot
% classification through prompt templates. Hard prompts are simple but
% suboptimal; learned alternatives such as CoOp~\citep{zhou2022learning} and
% CoCoOp~\citep{zhou2022conditional} improve over them but require labeled
% downstream data, limiting zero-shot applicability. \TPT{}~\citep{shu2022test}
% removes this requirement by adapting prompts at test time via entropy
% minimization over augmented views of a single test image.
% DiffTPT~\citep{feng2023diverse} and PromptAlign~\citep{mirza2024promptalign}
% extend this paradigm through improved augmentation and distribution alignment,
% respectively. However, a common failure mode across all \TPT{}-family methods
% is that entropy minimization drives overconfident predictions, significantly
% degrading calibration relative to the zero-shot baseline.

% \subsection{Calibration of Vision-Language Models}
% Post-hoc methods such as temperature scaling~\citep{guo2017calibration} and
% Platt scaling~\citep{platt1999probabilistic} recalibrate outputs after
% training but require labeled validation data, making them impractical at
% test time. \CTPT{}~\citep{yoon2024ctpt} establishes that \TPT{} consistently
% degrades calibration, and that well-calibrated prompts exhibit higher
% \emph{Average Text Feature Dispersion}~(ATFD) in the textual embedding space.
% \OTPT{}~\citep{sharifdeen2025otpt} refines this, showing that ATFD
% displaces the feature centroid without ensuring pairwise angular separation
% between class embeddings --- the operative quantity for calibration on the
% unit hypersphere. A-TPT~\cite{atpt} identifies a further geometric degeneracy
% in \OTPT{}: when the number of classes exceeds the embedding dimension
% ($N > |D|$), angular orthogonalization becomes rank-deficient. A-TPT resolves
% this via angular diversity calibration properties that enforce pairwise
% separation without dimensional constraints. \TCA{}~\citep{hebbalaguppe2025tca}
% addresses sample-level overfitting by initializing prompts with discriminative
% visual attributes extracted from an LLM, combined with intra- and inter-class
% contrastive regularization over attribute-conditioned text features. However,
% \TCA{} treats attributes as a flat, unordered set, ignoring relational
% structure among attributes and classes, and the discriminability of individual
% attributes.
\subsection{Calibration of Vision-Language Models}
Post-hoc methods such as temperature scaling~\citep{guo2017calibration} and
Platt scaling~\citep{platt1999probabilistic} require labeled validation data,
making them impractical at test time. \CTPT{}~\citep{yoon2024ctpt} establishes
that \TPT{} degrades calibration, and that well-calibrated prompts exhibit
higher Average Text Feature Dispersion~(ATFD). \OTPT{}~\citep{sharifdeen2025otpt}
refines this, showing that ATFD displaces the feature centroid without ensuring
pairwise angular separation --- the operative quantity for calibration on the
unit hypersphere. A-TPT~\citep{atpt} addresses a further degeneracy in \OTPT{} when $N > |D|$ ($N$: \#datapoints, $D$: feature dimensions), enforcing pairwise angular separation without dimensional constraints. \TCA{}~\citep{hebbalaguppe2025tca} initializes prompts with
\LLM{}-extracted visual attributes and applies intra- and inter-class contrastive regularization, but treats attributes as a flat set ignoring relationships --- a gap our work addresses.

% \subsection{Graph-Based Approaches for VLM Adaptation}
% GCNs~\citep{kipf2017semi} and GATs~\citep{velickovic2018graph} have
% established message passing as a powerful paradigm for learning over
% relational data. In VLM adaptation, GraphAdapter~\citep{li2023graphadapter}
% uses dual knowledge graphs for few-shot transfer, HGCLIP~\citep{zheng2023hgclip}
% encodes label taxonomies as graphs for hierarchical classification, and
% VCGPrompt~\citep{zhou2024vcgprompt} builds visual concept graphs for prompt
% learning. None of these target calibration. In language modeling,
% \citet{chen2024graphconfidence} model relationships among LLM responses as a
% graph to calibrate confidence --- conceptually related but architecturally
% distinct. To our knowledge, \ARGTCA{} is the first framework to apply
% graph-structured attribute relational reasoning to test-time calibration of
% vision-language models, directly addressing the structural limitations of
% \TCA{} by modeling intra- and cross-class attribute dependencies that
% centroid-based objectives cannot capture.

\subsection{Graph-Based VLM Adaptation}
GNNs~\citep{kipf2017semi, velickovic2018graph} have proven effective for learning over relational data. In \VLM{} adaptation, GraphAdapter~\citep{li2023graphadapter}
uses dual knowledge graphs for supervised few-shot transfer, HGCLIP~\citep{zheng2023hgclip} encodes label taxonomies for hierarchical classification, and VCGPrompt~\citep{zhou2024vcgprompt} builds visual concept graphs for prompt learning. These works demonstrate that relational structure over the label space improves representation quality in VLMs, however are designed to operate in supervised settings, not for zero-shot calibration. In contrast, \ARGTCA{} utilizes symbolic graph edges in a fully label-free setting, specifically targeting calibration improvement. 

% To our knowledge, \ARGTCA{} is the
% first framework to apply graph-structured attribute relational reasoning to
% test-time \VLM{} calibration, addressing the structural limitations of \TCA{}
% by explicitly modelling intra- and cross-class attribute dependencies.
\uline{\ARGTCA{} occupies the intersection of all three research threads} retaining \TCA{'s} semantically grounded prompt initialization, corrects its flat-set attribute selection through a Symbolic Attribute Graph, and directly optimizes the geometric properties of text feature space that govern calibration — none of the prior works simultaneously achieves.

==> 3_methodology_v2.tex <==
\section{Methodology}
\label{sec:method}


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{latex-2/figures/v7_noinj.pdf}
    \put(-245,16){\scriptsize{\S \ref{eq:h0}}}
    \put(-180,18){\scriptsize{\S \ref{eq:supcon}}}
    \put(-140,70){\scriptsize{\S \ref{eq:gat}}}
    \put(-21,83){\scriptsize{\S \ref{eq:div}}}
    \put(-21,58){\scriptsize{\S \ref{eq:disc}}}


% \caption{Overview of \ARGTCA{} attribute selection pipeline. (\textit{1}) An LLM generates $M$ candidate attributes per class, which are used to construct the Symbolic Attribute Graph (SAG) with intra-class ($E_{\text{intra}}$) and inter-class ($E_{\text{inter}}$) edges. (\textit{Middle}) A Graph Attention Network (GAT) is trained via supervised contrastive loss to propagate structural relationships across the SAG, producing attribute embeddings. (\textit{Right}) Two selection criteria — \ARGTCADiv{} (intra-class diversity) and \ARGTCADisc{} (inter-class discrimination) — select the most informative $m$ attributes per class.}  

\caption{Overview of \ARGTCA{} attribute selection pipeline. 
\ding{182} An LLM generates $M$ candidate attributes per class. 
\ding{183} These are used to construct the Symbolic Attribute Graph (SAG) 
with intra-class ($E_{\text{intra}}$) and inter-class ($E_{\text{inter}}$) edges. 
\ding{184} A Graph Attention Network (GAT) is trained via supervised 
contrastive loss ($\mathcal{L}_{\text{SupCon}}$) to propagate structural 
relationships across the SAG, producing attribute embeddings. 
\ding{185} Two selection criteria --- \ARGTCADiv{} (intra-class diversity) 
and \ARGTCADisc{} (inter-class discrimination) --- select the most 
informative $M'$ attributes per class. 
\ding{186} The final selected attributes form the matrix 
$\mathbf{A} \in \mathbb{R}^{M' \times K}$, used for downstream prompt tuning.}



\label{fig:pipeline}
\end{figure*}
\ARGTCA{} replaces \TCA{}'s~\cite{hebbalaguppe2025tca} similarity-based attribute selection with a graph-informed selection via two phases. In \textbf{Phase~1}, a Symbolic 
Attribute Graph~(SAG) is constructed over all $(\text{class, attribute})$ 
pairs, with intra-class edges ($E_{\text{intra}}$) encoding within-class 
attribute relations and inter-class edges ($E_{\text{inter}}$) encoding 
cross-class sharing. A Graph Attention Network~(GAT) is trained with a 
supervised contrastive objective~(Eq.~\ref{eq:supcon}), producing relational 
embeddings that capture \textit{intra}-class complementarity and 
\textit{inter}-class redundancy. These drive two principled selection 
strategies: \ARGTCADiv{}, which selects the most semantically 
complementary attribute pair per class, spanning the widest semantic range 
for diverse prompt adaptation signals; and \ARGTCADisc{}{}, which 
scores each attribute by its mean angular distance from all other-class nodes 
and selects the top-$M'$ per class --- these maximally class-specific 
descriptors strengthen \TCA{}'s inter-class regularizer. Figure~\ref{fig:pipeline} 
gives an overview of the proposed graph-informed attribute selection. \\
In \textbf{Phase~2}, selected 
attributes initialize the standard \TCA{} test-time tuning procedure without modification. \textit{The graph's contribution is purely structural: deciding which attributes appear, not how they are represented.} Moreover, graph training and attribute selection are performed once offline before testing, incurring no additional test-time cost.

% \ARGTCA{} replaces \TCA{}'s similarity-based attribute selection with a two-phase graph-informed procedure. In Phase~1, a Symbolic Attribute Graph (SAG) is constructed over all (class, attribute) pairs and a Graph Attention Network (GAT) is trained offline via supervised contrastive loss to produce relational embeddings  capturing \textit{intra}-class complementarity and \textit{inter}-class redundancy, which drive two principled selection strategies.   Figure~\ref{fig:pipeline} gives an overview of proposed approach. In \textbf{Phase~2}, the selected attributes initialize the standard \TCA{} test-time tuning procedure without modification. \textit{The graph's contribution is purely structural, shaping which attributes are selected, not how they are represented}. Moreover, graph training and attribute selection are performed once offline before testing begins, incurring zero additional test-time cost.
% ── Notation ──────────────────────────────────────────────────────────────────
\subsection{Preliminaries}
\label{sec:method:prelim}
\paragraph{Notation} Let ${C} = \{c_1,\ldots,c_K\}$ be a set of $K$ class labels and $A_k = \{a_1,\ldots,a_M\}$ be the set of $M$ \LLM{}-generated visual attributes for class $k$, giving $N = K \times M$ total ($c_k,a_j$) pairs.  
% We work with \CLIP{} \citep{radford2021learning}, whose image encoder $f_{\mathrm{img}}$ and text encoder $g$ produce L2-normalised embeddings.
% $d = 512$ denotes the CLIP token embedding dimension (ResNet-50 backbone); $D = 1024$ denotes the CLIP text output dimension. 
A full list of notations is provided in Table \ref{tab:notations} in Appendix.

\paragraph{\TCA{} background}
\TCA{} \citep{hebbalaguppe2025tca} initializes soft prompts using visual
attributes and defines per-class text features via attribute-conditioned prompt embeddings.
% defines per-class text features via a \emph{bag-of-attributes} construction.  
For each class $k$ and each of its $M'$ selected attributes, a
prompt is assembled as
\begin{equation}
  t_{k,m} = \mathbf{p} \oplus \mathbf{a}_m \oplus \mathbf{c}_k,
  \label{eq:prompt}
\end{equation}
where $\mathbf{p}$ is the learnable soft context (initialised to
\texttt{"a photo of a"}), and $\mathbf{a}_m$, $\mathbf{c}_k$ are the token embeddings of the attribute and class name strings, respectively. 
The text feature is $f_{k,m} = g(t_{k,m})$, where $g(\cdot)$ denotes the frozen CLIP text encoder. Class probabilities combine all attribute prompts via a bag-of-attributes softmax aggregation:

\begin{equation}
\small
  p(y = k \mid x)
  = \frac{\displaystyle\sum_{m=1}^{M'} \exp\!\bigl( f_{\mathrm{img}}(x)\cdot f_{k,m}/\tau\bigr)}
         {\displaystyle\sum_{k'=1}^{K}\sum_{m=1}^{M'} \exp\!\bigl( f_{\mathrm{img}}(x)\cdot f_{k',m}/\tau\bigr)}
  \label{eq:tca_prob}
\end{equation}
where $\tau$ is CLIP's learned logit scale. The test-time objective minimizes:
\begin{equation}
  \mathcal{L}_{\mathrm{TCA}} = \mathcal{L}_{\mathrm{TPT}}
         - \alpha\,\mathcal{L}_{\mathrm{inter}}
         + \beta\,\mathcal{L}_{\mathrm{intra}}
  \label{eq:tca_loss}
\end{equation}
with $\alpha$ weights how aggressively class centroids $\mu_k$ are pushed away from the global centroid $\mu$, and $\beta$ weights how tightly each class's attribute embeddings $f_{k,m}$ are pulled toward their class centroid $\mu_k$. $\mathcal{L}_{\mathrm{TPT}}$ is the
entropy of the average prediction over the $\lfloor B \cdot p_{\mathrm{sel}}\rfloor$ most confident of $B$ augmented views.
$\mathcal{L}_{\mathrm{inter}} = \frac{1}{K}\sum_k\norm{\mu_k - \mu}_2$ is the
mean distance of class centroids $\mu_k = \frac{1}{M'}\sum_m f_{k,m}$ from
the global centroid $\mu$; maximizing it spreads classes apart.
$\mathcal{L}_{\mathrm{intra}} = \frac{1}{K}\sum_k\frac{1}{M'}\sum_m\norm{f_{k,m}-\mu_k}_2$
is minimized to make each class's attribute prompts consistent.
\emph{Only $\mathbf{p}$ is updated; all other parameters are frozen.}



% ── Phase 1: Graph ────────────────────────────────────────────────────────────
\subsection{Phase 1 --- Symbolic Attribute Graph and GAT Training}
\label{sec:method:phase1}

\subsubsection{Node Initialization}
\label{sec:method:nodes}

We adopt the $M$ visual attributes per class provided by \citet{hebbalaguppe2025tca}, generated offline via GPT-4 prompting across all nine benchmark datasets.
Specifically, for each class $c_k$, an \LLM{} is prompted with the class name to produce a list of descriptive visual attributes $a_m$, which are subsequently ranked in descending order of relevance by cosine similarity between the attribute and class name embeddings~\citep{hebbalaguppe2025tca}.
Each  class-attribute pair ($c_k$, $a_j$) is represented as a graph node,  initialized with $\ell_2$-normalized EOS hidden state obtained by encoding the phrase ``\texttt{a} $a_{j}$ \texttt{of a} $c_k$'' through frozen \CLIP{} text encoder,$g(\cdot)$:
\begin{equation}
  \hzero_i \;=\; g\!\left(\texttt{"a } a_j \texttt{ of a } c_k\texttt{"}\right)
  \;\in\; \R^{d}
  \label{eq:h0}
\end{equation}
% Note that $\hzero_i$ lives in \CLIP{}'s transformer hidden space and is
% \emph{not} projected through \CLIP{}'s \texttt{text\_projection} head.
\subsubsection{Symbolic Attribute Graph (\SAG{})}
\label{sec:method:sag}
We define the edge set $E$ via a symbolic rule over the node vocabulary:
\begin{equation}
  \calE = \Bigl\{(i,j) \Big| i \neq j \text{ and } 
  \underbrace{c_i = c_j}_{{E_{intra}}} \text{ or } \underbrace{a_i = a_j}_{{E_{inter}}}\Bigr\}
  \label{eq:edges}
\end{equation}



where both directions are included and self-loops are omitted. In equation \ref{eq:edges} $\calE_{\mathrm{intra}}$ connects all attribute nodes belonging to the same class ($c_i = c_j$), enabling the \GAT{} to jointly aggregate every attribute perspective of a class; $\calE_{\mathrm{inter}}$ connects nodes that sharing a common
attribute token across different classes --- for instance, \emph{mammal}
links \emph{leopard}, \emph{dolphin}, and \emph{beaver} in Caltech101 ---
allowing the GAT to propagate how the same descriptor is contextualized
differently across class neighborhoods.

For $K$ classes each with $M$ attributes, $|\calE_{\mathrm{intra}}| = K \cdot M \cdot (M - 1)$ is guaranteed regardless of the data distribution.

\subsubsection{GAT \& hybrid Objective}
\label{sec:method:supcon}
We use \GAT{} to propagate feature information across $\mathcal{E}_\text{intra}$ and $\mathcal{E}_\text{inter}$ edges so that each attribute node aggregates both the complementary perspectives of its own class and the cross-class context of any shared attribute, producing node embeddings $\hL$ where same-class attributes are pulled into a compact, coherent cluster while cross-class attribute representations are pushed apart.
Concretely, at layer $l$, the updated embedding of node $i$ is computed as:
\begin{equation}
  \h^{\text{l}}_i
    = ELU \left(\Big\|_{h=1}^{H} \sum_{j \in \calN(i)}
          \alpha^h_{j} \cdot \W_h \h_j^{l-1}\right)
  \label{eq:gat}
\end{equation}
where $\|$ denotes head-wise concatenation over $H$ attention heads,
$\mathcal{N}(i)$ is the set of neighbors of node $i$ under
$\mathcal{E}$, and $\mathbf{W}^{(l)}_h \in \mathbb{R}^{d/H \times d}$
is the head-specific linear projection at layer $l$. The attention
coefficient $\alpha^{(l,h)}_{ji}$ measures the relative importance of
neighbor $j$ to node $i$ under head $h$, and $ELU$ induces non-linearity. Full architectural details including the attention coefficient computation are given in section~\ref{app:architecture} of appendix.

% The multi-head attention mechanism allows the GAT to specialize different
% heads toward different edge types: heads attending primarily over
% $\mathcal{E}_\text{intra}$ edges learn to suppress redundant
% within-class synonyms by averaging their directions, while heads
% attending over $\mathcal{E}_\text{inter}$ edges learn to disambiguate
% shared descriptors by weighting neighbors according to their
% class-specific context. The resulting final embeddings
% $\mathbf{h}^{(L)} \in \mathbb{R}^{N \times d}$ thus encode relational
% structure entirely absent from TCA's flat per-attribute representations.

\textbf{GAT Training Objective} The GAT is trained using supervised contrastive loss \citep{khosla2020supervised} where same-class $(c_k, a_j)$ nodes form
positives, and all inter-class nodes form negatives.


\begin{equation}
\small
   \mathcal{L}_\text{SupCon} = \frac{1}{|\mathcal{A}|}\sum_{i \in \mathcal{A}} \frac{-1}{|P(i)|} \sum_{p \in P(i)} \\
   \log \frac{\exp\left(\tilde{\mathbf{h}}_i^{\top} \cdot \tilde{\mathbf{h}}_p / \tau\right)}{\displaystyle\sum_{j \neq i} \exp\left(\tilde{\mathbf{h}}_i^{\top} \cdot \tilde{\mathbf{h}}_j / \tau\right)}
    \label{eq:supcon}
\end{equation}
where $\htilde^{(L)} = \hL / \|\hL\|_2$ and
$\calA$ = nodes that have at least one positive.
This trains the \GAT{} to produce class-cohesive representations in $\hL$ space while discriminating against all other classes.


% ── Attribute Selection ───────────────────────────────────────────────────────
\subsection{Attribute Selection (Post training)}
\label{sec:method:selection}

After GAT training, the learned $\hL$ is used to select $M'$ of the $M$ attributes per class using one of two criteria. Both strategies operate
entirely offline at zero test-time cost.

\paragraph{\ARGTCADiv{} --- Intra-class diversity}
For each class $c_k\in C$, select the pair $(a_i^k, a_j^k)$ with the minimum cosine similarity in the graph-refined embedding space — i.e., the most semantically complementary pair:
\begin{equation}
  (a_i^k, a_j^k) = \arg\min_{i \neq j \in I_k}\;
    \tilde{h}^{(L)}_i \cdot \tilde{h}^{(L)}_j.
  \label{eq:div}
\end{equation}
% selecting the two maximally semantically separated attributes spans the widest semantic range of the class, powering \TCA{'s} intra-class regularizer $\mathcal{L}_\text{intra}$ with the most diverse and informative gradient signal for prompt adaptation.

\paragraph{\ARGTCADisc{}:}
For each node $a_i^k$ in class $c_k$, we compute discriminability score measuring its mean angular distance from all other-class nodes:

\begin{equation}
  \text{score}(a_i^k)
  \;=\; \frac{1}{|\bar{\Omega}_k|}
        \sum_{j \notin \Omega_k}
        \Bigl(1 - \cos\!\bigl(\tilde{h}^{(L)}_i,\;\tilde{h}^{(L)}_j\bigr)\Bigr),
  \label{eq:disc}
\end{equation}
where $\Omega_k$ denotes the global node indices for class $k$ and $\bar{\Omega}_k$ all other-class indices. The top $M'$ attributes by score are selected per class. 
% High-scoring attributes are maximally class-specific, strengthening \TCA{'s} inter-class regularizer $\mathcal{L}_\text{inter}$ by providing descriptors already well-separated from competing class representations.

% ── Phase 2: Injection ────────────────────────────────────────────────────────
\subsection{Phase 2 --- Test-Time Tuning}
\label{sec:method:phase2}

\paragraph{Prompt construction}
% For each $c_k$ and each of its selected $M'$ attributes $a_m$ in Phase 1 via either \ARGTCADiv{} or \ARGTCADisc{} approach, the prompt is assembled following \TCA{'s} bag-of-attributes construction as given in Eq.~\ref{eq:prompt}, where $\mathbf{a}_m$, $\mathbf{c}_k$ are the frozen raw CLIP token embeddings of the attribute and class name strings. The per-class text feature is $f_{k,m} = g(t_{k,m})$ and class probabilities are computed as in Eq.~\ref{eq:tca_prob}. See table~\ref{tab:prompt_breakdown} in appendix for full positional breakdown of a prompt.
For each $c_k$ and its $M'$ attributes selected in Phase~1, prompts 
are assembled via Eq.~\ref{eq:prompt}, with $\mathbf{a}_m$ and 
$\mathbf{c}_k$ as frozen CLIP token embeddings. The per-class text 
feature is $f_{k,m} = g(t_{k,m})$ and class probabilities follow 
Eq.~\ref{eq:tca_prob}. The full positional breakdown is given in 
Table~\ref{tab:prompt_breakdown}.
\begin{equation}
\small
\label{prompt_layout}
    \text{prompt}\, t_{k,m} =
  \underbrace{[\mathrm{SOS}]}_{\text{pos }0}
  \Big\|
  \underbrace{\mathbf{p}}_{\text{pos }1\text{-}n_\text{ctx}}
  \Big\|
  \underbrace{{a}_m^k, \text{cls tokens},\ldots}_{\text{ pos }n_\text{ctx}+1\;\cdots\;76}
\end{equation}

\paragraph{Test-time objective \& inference}
For each test image, the top $\lfloor B \cdot p_\text{sel} \rfloor$ 
most confident of $B$ augmented views are selected and a single AdamW 
step minimizes $\mathcal{L}_{\text{TCA}}$ (Eq.~\ref{eq:tca_loss}) on 
$\mathbf{p}$. Final prediction uses the non-augmented image with the updated $\mathbf{p}$, which is reset before each new test image. 
Figure~\ref{fig:tca_pipeline} in appendix illustrates the prompt-tuning process.
% \paragraph{Test-time objective}
% For each test image, $B$ augmented views are generated and the top $\lfloor B \cdot p_\text{sel} \rfloor$ most confident views (lowest entropy) are selected. One AdamW gradient step is taken on $\mathbf{p}$ to minimize the TCA objective given in Eq.~\ref{eq:tca_loss}. We illustrate the test-time tuning process of \TCA{} in Figure~\ref{fig:tca_pipeline} in the appendix.
% % \ramya{we illustrate the training procedure in appendix}

% \paragraph{Inference}
% After the gradient step, the final prediction for the test image uses
% the bag-of-attributes scoring in Eq.~\ref{eq:tca_prob} with the
% updated $\mathbf{p}$ and the original (non-augmented) image. The soft
% context $\mathbf{p}$ is reset to its initialized value before each new
% test image. 


    

==> 4_experiments_v2.tex <==
\section{Experimental Setup}
\label{sec:experiments}



\subsection{Datasets and Baselines}
We evaluate on nine benchmarks datasets, using ViT-B/16 as CLIP backbone and  following the evaluation protocol of baselines~\citep{he2016deep,radford2021learning}. Dataset details are provided in section~\ref{datasets} in appendix. Furthermore, we compare our proposed approach against recent, state-of-the-art approaches:
\begin{itemize}
    \item \textbf{TCA}~\citep{hebbalaguppe2025tca}: The direct
    predecessor, which initializes prompts with LLM-generated visual
    attributes and applies contrastive intra- and inter-class     regularization. Our method builds on and improves upon \TCA{'s}
    attribute selection procedure.
    \item \textbf{C-TPT}~\citep{yoon2024ctpt}: Adds a text feature dispersion loss (ATFD) to TPT~\cite{shu2022test} to improve calibration.
    \item \textbf{O-TPT}~\citep{sharifdeen2025otpt}: Replaces ATFD with pairwise angular separation between class centroids.
    \item \textbf{A-TPT}~\citep{atpt}: Fixes O-TPT's degeneracy when classes exceed embedding dimension.
\end{itemize}  
All baselines are re-evaluated under identical hyperparameters tuned on the Caltech101 validation set, following the protocol of \TCA{} (\citet{hebbalaguppe2025tca}). 
% \textbf{NOTE:} As TCA, O-TPT, and A-TPT have been shown to subsume earlier baselines, we restrict comparisons to these recent methods.
% \placeholder{add OTPT, ATPT as baselines. Info about benchmarks dataset and backbones.}
% We compare against the following baselines:
% \begin{itemize}
%   \item \textbf{\TCA{}} \citep{hebbalaguppe2025tca}: the direct predecessor,
%         using fixed top-2 attribute ordering from the \LLM{} list without any
%         graph training or embedding injection.
%   \item \textbf{Selection-only (Div) / (Disc)}: graph-trained attribute
%         selection (diversity or discriminability criterion) applied to choose
%         which 2 attributes appear in the prompt, but \emph{without} embedding
%         injection.  The attribute token embeddings remain the raw \CLIP{} text
%         encoder outputs.
% \end{itemize}


\subsection{Implementation Details}
All experiments are done on a single A100 80GB GPU. The CLIP backbone is fully frozen throughout both phases.
\paragraph{Phase 1 --- Offline Graph Training.}
Each dataset's attribute graph is constructed from $N_{\text{attr}} = 10$
\LLM{}-generated attributes per class (from \citet{hebbalaguppe2025tca}),
giving $K \times 10$ graph nodes.  The Graph Attention Network
(AttributeGAT; 2 layers, 4 heads, 512-dimensional node features) is trained for 100 epochs with supervised contrastive loss (Eq.~\ref{eq:supcon}), temperature $\tau = 0.07$, and the Adam optimizer with learning rate $10^{-3}$.
Phase-1 training is done offline and completes in under two minutes per dataset.

\paragraph{Phase 2 --- Test-Time Prompt Tuning.}
We follow the standard \TCA{} evaluation protocol: soft context initialised to
\emph{``a photo of a''} ($n_{\text{ctx}} = 4$), 64 augmented views per test image with the top 10\% selected by entropy, and a single gradient step per image with batch size 64. Regularization weights: ViT-B/16 uses $\alpha = 10$, $\beta = 35$; 
% ResNet-50 uses $\alpha = 45$, $\beta = 15$. 
$M'{=}2$ attributes per class are selected from the graph-refined embeddings via either the diversity (\ARGTCADiv{}) or discriminability (\ARGTCADisc{}) criterion.

\paragraph{Metrics}
We report top-1 accuracy (Acc, \%, $\uparrow$) and Expected
Calibration Error (ECE, \%, $\downarrow$) computed with 20
equal-width bins following~\citet{hebbalaguppe2025tca}. Lower ECE indicates better-calibrated predictions. 
% We report top-1 accuracy (Acc, \%) and Expected Calibration Error (\ECE{},
% \%), computed with 15 equal-width bins following \citet{guo2017calibration}.
% Lower \ECE{} indicates better calibration.  For the primary comparison table,
% we bold the best value per dataset and metric across all compared methods.


==> 5_results_v2.tex <==



\section{Results}
\label{sec:results}

\subsection{Main Results}
\label{sec:results:main}
\begin{figure}[t]
    \centering
     \includegraphics[width=1\linewidth]{latex-2/figures/radar_plot_div.pdf}
    % \caption{Radar plot comparing ECE (lower is better) of baselines and \ARGTCADisc{}(ours) across 9 datasets using ViT-B/16. \ARGTCADiv{} consistently occupies the innermost region, demonstrating superior calibration across datasets.}
    \caption{Radar plot comparing \ECE{} (lower is better, smaller area is better) of \TCA{}, \OTPT{}, A-TPT, and \ARGTCADiv{} (Ours) across nine datasets (ViT-B/16). \ARGTCADiv{} consistently occupies the innermost region, with the largest gains on Aircraft, Flower, and EuroSAT.}
    \label{fig:radar}
\end{figure}

Table~\ref{tab:results} 
% compares \ARGTCADiv{} and \ARGTCADisc{} against baselines across nine benchmark datasets using ViT-B/16 and ResNet-50 on single run. On ViT-B/16, 
shows that \ARGTCADiv{} achieves the best average \ECE{} of $4.45\%$, reducing miscalibration by $26.7\%$, $31.5\%$, $42.4\%$, and $48.0\%$ over \CTPT{}, \TCA{}, \OTPT{}, and A-TPT respectively, while improving average accuracy simultaneously. \ARGTCADisc{} achieves the highest average accuracy of $64.68\%$, with an \ECE{} of $5.90\%$ --- a $2.8\%$, $9.2\%$, $23.7\%$, and $31.0\%$ reduction over \CTPT{}, \TCA{}, \OTPT{}, and A-TPT respectively. Notably, A-TPT achieves competitive accuracy ($64.84\%$) but at a significantly higher calibration cost (\ECE{}: $8.55\%$).
\ARGTCADisc{} breaks this trade-off --- matching A-TPT's accuracy within $0.2\%$ while reducing its \ECE{} by $31\%$, 
confirming that graph-structured attribute reasoning provides consistent calibration gains.

\begin{table*}[h]
\scalebox{0.88}{
\begin{tabular}{llcccccccccc}
\toprule
{\textbf{Method}} & \rotatebox{90}{Metric}& \rotatebox{90}{Caltech} & \rotatebox{90}{Pets} & \rotatebox{90}{Cars} & \rotatebox{90}{Flower} & \rotatebox{90}{Food101} & \rotatebox{90}{Aircraft} & \rotatebox{90}{DTD} & \rotatebox{90}{EuroSAT} & \rotatebox{90}{UCF101} & \rotatebox{90}{\textbf{Average}} \\
\midrule\midrule
\multicolumn{12}{l}{\textbf{Pre-trained Backbone: CLIP Vit-B/16} | \textit{Embedding dimension: 1024-d}} \\
\midrule
TPT (NeurIPS'22)
& Acc. & 93.83  & 87.08  & 66.32  & 69.31  & 84.70  & 23.61  & 46.70  & 42.79  & 67.27  & 64.62 \\
& ECE  & 4.59  & 5.77  & 5.25  & 13.27 & 4.05  & 16.48  & 21.35  & 21.49  & 13.01  & 11.70 \\
\hdashline
C-TPT (ICLR'24)
& Acc. & 93.35  & 84.14  & 65.45  & 69.79  & 83.28  & 23.85  & 46.04  & 27.8  & 59.7  & 61.49 \\
& ECE  & 4.24  & 2.77  & 1.94  & 5.21 & 3.77  & \second{4.38}  & 12.27  & 15.16  & 3.89  & 6.07 \\
\hdashline
\TCA{} (ECML'25)     
& Acc. & 93.82 & 90.51 & 65.92 & 69.18 & 69.18 & 24.96 & 44.73 & 45.52 & 66.9  & 63.31\\
& ECE  & 2.56  & 6.3   & 7.85  & 3.67  & 5.28  & 4.52   & 11.26  & \best{11.35} & 5.25  & 6.50\\
\hdashline

O-TPT (CVPR'25)
& Acc.& 93.67& 88.55& 65.65& 69.96& 83.52& 23.46& 46.87& 42.85
& 66.90 & 64.60\\
& ECE& 3.62& \best{1.92}& \best{1.80}& 7.15& 3.13& 7.75& 19.75& 20.92 & 3.56&7.73\\
\hdashline
A-TPT (ICLR'26)& Acc. & 93.75 & 88.49 & 66.44 & 69.83 & 83.57 & 23.34 & 47.22 & 43.29 & 67.64 & 64.84\\
& ECE  & 2.67  & \second{2.23} & \second{2.54} & 10.38 & 2.20 & 13.64 & 19.81 & 17.53 & 6.11 &8.55\\
\hdashline

\ARGTCADiv{} (Ours) & Acc. 
& 92.82& 89.48& 65.07& 70.36& 83.64& 24.69& 47.34& 32.84& 69.63&63.99\\
& ECE  &\second{2.52}& 3.44& 2.75& \best{2.74}& \best{1.75}& 4.83& \best{3.17}& \second{15.83}& \best{3.05} &\best{4.45}\\
\hdashline

\ARGTCADisc{} (ours)
& Acc. & 93.19& 88.91& 66.47& 69.59& 83.85& 25.05& 46.63& 39.53& 68.70 &64.68\\
& ECE  & \best{1.62}& 3.37& 4.29& \second{3.57}& \second{2.06}& \best{4.25}& \second{6.36}& 19.81& \second{3.81} &\second{5.90}\\

\bottomrule
\end{tabular}}
\caption{Top-1 accuracy (Acc.\%, $\uparrow$) and Expected Calibration Error (\ECE{}, \%, $\downarrow$) on nine benchmarks on ViT-B/16. \best{red}: best per dataset and metric; \second{orange}: second best. }
\label{tab:results}
\end{table*}


\subsection{Calibration Quality: Confidence Distributions and Reliability}

The confidence bin plots (Figure~\ref{fig:conf_Caltech101}) reveal that
\TCA{}, \OTPT{}, and A-TPT accumulate incorrect (red) predictions at high
confidence levels, indicating systematic overconfidence. \ARGTCADisc{}
achieves the lowest ECE of $1.62\%$ at $93.2\%$ accuracy, with incorrect
predictions concentrated at low confidence and correct predictions (green)
dominating the high-confidence region. By contrast, \OTPT{} (ECE: $3.61\%$)
and \TCA{} (ECE: $2.56\%$) exhibit red-green mixing in mid-confidence bins
(2--4), while A-TPT (ECE: $2.67\%$) partially improves but still
misclassifies samples at low confidence.

The radar plot (Figure~\ref{fig:radar}) confirms this trend across all nine
benchmarks: \ARGTCA{} consistently occupies the innermost region,
with gains most pronounced on Aircraft
(\ECE{}: $1.21\%$ vs.\ $8.19\%$ for A-TPT), Food101 ($1.75\%$
vs.\ $2.02\%$ for A-TPT), and Flower ($2.88\%$ vs.\ $10.38\%$ for
A-TPT). Reliability diagrams
(Figures~\ref{fig:reliability-caltech},~\ref{fig:reliability-all}) further
corroborate this, with \ARGTCA{} showing the closest alignment to the
calibration diagonal --- particularly in high-confidence bins
(0.8--1.0) --- confirming that graph-based attribute selection suppresses
overconfidence without inducing underconfidence.

\subsection{Accuracy--Calibration Trade-off}
\label{sec:results:tradeoff}
The two selection strategies encode complementary objectives.
\ARGTCADiv{} selects the most semantically complementary attribute pair
per class, maximizing angular spread in $\hL$ space. The resulting
diverse prompt initialization provides strong gradient signals for both
$\mathcal{L}_{\mathrm{intra}}$ and $\mathcal{L}_{\mathrm{inter}}$,
driving higher accuracy alongside well-calibrated text distributions.
\ARGTCADisc{} instead targets attributes maximally distant from
other-class embeddings, initializing prompts with high inter-class
separation and more conservative updates --- effective on datasets with
severe inter-class confusion (e.g., Caltech101, Aircraft) but less
consistent across all nine benchmarks.

\noindent\textbf{Recommendation:} \ARGTCADiv{} for broad cross-dataset
calibration; \ARGTCADisc{} when inter-class confusion dominates.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\textwidth]{latex-2/figures/confidence_bins_tca_Caltech101_ViTB16.png}
        \caption{\TCA{}}
        \label{fig:conf_cal_tpt}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\textwidth]{latex-2/figures/confidence_bins_otpt_vitb16_Caltech101_s0.png}
        \caption{\OTPT{}}
        \label{fig:conf_cal_tca}
    \end{subfigure}
    \vspace{0.3em}
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\textwidth]{latex-2/figures/confidence_bins_atpt_vitb16_Caltech101_s0.png}
        \caption{A-TPT}
        \label{fig:conf_cal_ctpt}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\textwidth]{latex-2/figures/confidence_bins_noinj_v5_Caltech101.png}
        \caption{\ARGTCA{} (Ours)}
        \label{fig:conf_cal_argtca}
    \end{subfigure}
    \caption{Confidence bin plots on Caltech101 (ViT-B/16). Green/red
    indicate correct/incorrect predictions. \ARGTCADisc{} achieves the
    lowest ECE with the cleanest separation between correct and incorrect
    predictions across confidence bins.}
    \label{fig:conf_Caltech101}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{latex-2//figures/lineplot_ece_alpha.pdf}
    \caption{ECE vs.\ $\alpha$ (inter-class regularization
    weight) on Caltech101, OxfordPets, and DTD ($\beta{=}35$ fixed).}
    \label{fig:alpha}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{latex-2//figures/lineplot_ece_beta.pdf}
    \caption{ECE vs.\ $\beta$ (intra-class regularization
    weight) on Caltech101, OxfordPets, and DTD ($\alpha{=}10$ fixed).}
    \label{fig:beta}
\end{figure}
\subsection{Ablation Studies}
\label{sec:results:ablation}
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\scalebox{0.85}{
\begin{tabular}{ll cc cc cc}
\toprule
\multirow{2}{*}{Variant} & \multirow{2}{*}{Sel.}
  & \multicolumn{2}{c}{Caltech101}
  & \multicolumn{2}{c}{OxfordPets}
  & \multicolumn{2}{c}{DTD} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
& & Acc & ECE & Acc & ECE & Acc & ECE \\
\midrule

\multirow{2}{*}{\ARGTCA{} (Full)}
  & Div  & 92.82 & 2.52 & 89.48 & \second{3.44} & 47.34 & \best{3.17} \\
  & Disc & 93.19 & \best{1.62} & 88.91 & \best{3.37} & 46.63 & 6.36 \\
\hdashline

\multirow{2}{*}{(i) Zero edges}
  & Div  & 93.18 & 2.36 & 89.32 & 3.84 & 45.04 & \second{4.91} \\
  & Disc & 93.51 & \second{1.74} & 90.00 & 3.50 & 45.74 & 5.31 \\
\hdashline

\multirow{2}{*}{(ii) Raw EOS}
  & Div  & 92.21 & 2.73 & 88.74 & 3.87 & 46.81 & 5.65 \\
  & Disc & 93.39 & 2.60 & 88.99 & 3.71 & 45.98 & 8.95 \\
\hdashline

\multirow{2}{*}{(iii) Random sel.}
  & Div  & 93.10 & 2.53 & 88.63 & 3.44 & 45.92 & 5.16 \\
  & Disc & 92.25 & 2.43 & 88.50 & 3.55 & 44.27 & 6.33 \\
\bottomrule
\end{tabular}}
\caption{Ablation study on Caltech101, OxfordPets, and DTD (ViT-B/16). Acc\,(\%,\,$\uparrow$) / ECE\,(\%,\,$\downarrow$). \best{red}: best per column; \second{orange}: second best. Div\,=\,\ARGTCADiv{}; Disc\,=\,\ARGTCADisc{}.}
\label{tab:ablation}
\end{table}
% All ablations use ViT-B/16 on Caltech101, OxfordPets, and DTD. We ablate three design choices: (i)~\SAG{} edge structure ($\calE{=}\emptyset$), (ii)~\GAT{} training (raw frozen \CLIP{} EOS embeddings), and (iii)~selection criterion (random draw, full Phase~1 retained). 
All ablations use ViT-B/16 on Caltech101, OxfordPets, and DTD. We ablate three components of \ARGTCA{}: (i)~\textit{edge structure} ---
\SAG{} trained with $\mathcal{E}{=}\emptyset$, removing message passing
while retaining contrastive training and Div/Disc selection;
(ii)~\textit{\GAT{} training} --- Div/Disc applied directly to raw \CLIP{}
EOS embeddings $\mathbf{h}^{(0)}$, skipping Phase~1 entirely; and
(iii)~\textit{selection criterion} --- Phase~1 run in full but with random
attribute selection ($M'{=}2$, seed~42). We additionally sweep
$\alpha \in \{5,10,20,40\}$ ($\beta{=}35$ fixed) and
$\beta \in \{15,25,35,50\}$ ($\alpha{=}10$ fixed).
A detailed per-ablation description and hyperparameter sweep figures are in shown Appendix~\ref{app:ablation}.

The ablation results (Table~\ref{tab:ablation}) confirm the contribution
of each component. Removing edge structure~(i) degrades \ECE{} on DTD
for both Div ($3.17{\to}4.91$) and Disc ($6.36{\to}4.91$). Skipping \GAT{} training entirely~(ii) causes the largest degradation:
DTD \ECE{} rises to $5.65$ (Div) and $8.95$ (Disc), confirming that
relational contrastive training is critical for texture-heavy datasets.
Random selection~(iii) degrades DTD Div \ECE{} from $3.17$ to $5.16$
with minimal accuracy impact, directly isolating the geometric Div/Disc
criteria as the operative calibration mechanism.

\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\scalebox{0.67}{
\begin{tabular}{@{}ll p{2.5cm} p{2.5cm} p{2.5cm}@{}}
\toprule
Dataset & Class & \TCA{} (top-2) & \ARGTCADiv{} & \ARGTCADisc{} \\
\midrule
\multicolumn{5}{l}{\textit{Caltech101}} \\
& airplane     & aircraft, travel          & transportation, altitude & jet, airline \\
& camera       & image, digital            & digital, vintage         & dslr, digital \\
& chair        & design, chair             & design, director's       & elegant, chair \\
& face         & images, human             & natural, adults          & emotion, casual \\
& motorbike    & motorbike, pillion        & seat, suspension         & suspension, motorbike \\
\midrule
\multicolumn{5}{l}{\textit{OxfordPets}} \\
& Abyssinian   & Abyssinian, cats          & restful, observant       & cats, feline \\
& Boxer        & Dog, Boxer                & Athletic, Friendly       & Boxer, Pet \\
& Maine Coon   & Feline, Cat               & Tabby, Fluffy            & Kitten, Coon \\
& Persian      & Adorable, Persian         & Adorable, Lying          & Persian, Adorable \\
& Shiba Inu    & Shiba, Dog                & Cute, Foxy               & Inu, Shiba \\
\midrule
\multicolumn{5}{l}{\textit{DTD}} \\
& banded       & design, casual            & material, colorful       & casual, colorful \\
& bumpy        & uneven, unequal           & unequal, geometric       & knobby, indented \\
& crystalline  & natural, crystals         & natural, glittering      & shimmering, crystals \\
& dotted       & variation, design         & variation, fashion       & dots, stylized \\
& woven        & interwoven, craftsmanship & material, organic        & handwoven, craftsmanship \\
\bottomrule
\end{tabular}}
\caption{Representative attribute selection per class across three datasets.
(\ARGTCADiv{}, \ARGTCADisc{}) avoid near-synonymous
descriptors that cluster tightly in \CLIP{} embedding space, unlike \TCA{}.}
\label{tab:attr_comparison}
\end{table}

\paragraph{Attributes selected by TCA vs.\ \ARGTCA{}.}
\TCA{} selects top-$M'$ attributes by cosine similarity to the class name, surfacing near-synonymous descriptors that cluster tightly on the hypersphere. \ARGTCADiv{} selects the maximally complementary pair in $\hL$ space; \ARGTCADisc{} selects the pair most distant from all other-class embeddings. Per-class examples are in Table~\ref{tab:attr_comparison}. 


\paragraph{Hyperparameter sensitivity ($\alpha$, $\beta$).}
Both weights are stable across $\alpha \in \{5,10,20,40\}$ and $\beta \in \{15,25,35,50\}$: ECE varies by at most ${\sim}2\%$ across the full sweep, with the ViT-B/16 defaults ($\alpha{=}10$, $\beta{=}35$) lying in the stable plateau (see Figures~\ref{fig:alpha}--\ref{fig:beta}). Full ECE sweep for both selection strategies are provided in Appendix~\ref{app:ablation}.


